Automated forest inventory: analysis of high-density airborne LiDAR point clouds with 3D deep learning

Detailed forest inventories are critical for sustainable and flexible management of forest resources, to conserve various ecosystem services. Modern airborne laser scanners deliver high-density point clouds with great potential for fine-scale forest inventory and analysis, but automatically partitioning those point clouds into meaningful entities like individual trees or tree components remains a challenge. The present study aims to fill this gap and introduces a deep learning framework, termed ForAINet, that is able to perform such a segmentation across diverse forest types and geographic regions. From the segmented data, we then derive relevant biophysical parameters of individual trees as well as stands. The system has been tested on FOR-Instance, a dataset of point clouds that have been acquired in five different countries using surveying drones. The segmentation back-end achieves over 85% F-score for individual trees, respectively over 73% mean IoU across five semantic categories: ground, low vegetation, stems, live branches and dead branches. Building on the segmentation results our pipeline then densely calculates biophysical features of each individual tree (height, crown diameter, crown volume, DBH, and location) and properties per stand (digital terrain model and stand density). Especially crown-related features are in most cases retrieved with high accuracy, whereas the estimates for DBH and location are less reliable, due to the airborne scanning setup.

==> thebigtable.tex <==
\newpage
{
\tiny
\begin{ThreePartTable}
\begin{TableNotes}
\item[a] Partly available.
\item[b] Contact the author.
\item[c] No pointwise instance ID.
\item[d] Incorporated in CloudCompare software.
\end{TableNotes}

\begin{landscape}
\begin{xltabular}{\textwidth}{p{4.5cm}p{6.5cm}p{6.5cm}p{2.5cm}}
\captionsetup{justification=centering}
\caption{Representative methods for single and multiple tasks to segment trees based on point clouds}
\label{tab:RepresentativeMethods}\\
\toprule
Tasks &
  Highlights of methods &
  Remarks &
  References \\* \midrule
\endfirsthead
%
\multicolumn{4}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\toprule
Tasks &
  Highlights of methods &
  Remarks &
  References \\* \midrule
\endhead
%
\bottomrule
\endfoot
%
\endlastfoot
%
Single task: individual tree detection &
   &
  Main output is tree location. &
   \\
\hspace*{4em}Locate stem center &
  (1) Connected component segmentation of stem points. &
  Data collected by TLS in Evo, Finland and Beijing, China; Other output is DBH; Data open\tnote{a}; Code not open. &
  \citep{Zhang2019Jan16ANovel} \\
 &
  (2) Intensity-based point clustering per scanline. &
  Data collected by MLS and ALS in southern Sweden; Other outputs are DBH, stem profiles and stem volume; Data not open; Code not open. &
\citep{PaulaPires2022Mar18Individual} \\
 &
  (3) Multiple 2D raster based on height sections. &
  Data collected by DLS and TLS in Aichi prefecture, Japan; Other output is tree height; Data not open; Code not open. &
  \citep{Zhang2023Feb2ATree} \\
\hspace*{4em}Locate crown center &
  (4)Find local maxima in a CHM as initial tree locations, and accurately identify the tree top positions by combining a raster-based tree crown delineation approach with information from the DSM and DTM. &
  Data collected by ALS in Wellington, New Zealand; Other output is tree crown delineation; Data open; Code open. &
  \citep{Zoerner2018Nov13LiDAR} \\
 &
  (5) Locate tree position at the clustering center of higher points within a spatial neighborhood, and detect the center by a location-based recursive algorithm. &
  Data collected by ALS in simulated forest, Milwaukee, Wisconsin, U.S. and Denton, Texas, U.S.; Data not open; Code not open. &
  \citep{Liu2021Mar6Individual} \\
Single task: individual tree crown segmentation &
   &
  Main output is individual tree crown delineation or crown width. &
   \\
\hspace*{4em}DSM or CHM based &
  (6) Height raster image based graph partition. &
  Data collected by ALS in Vernon Parish, Louisiana, U.S.; Data not open; Code not open. &
  \citep{Strimbu2015Mar18graph} \\
 &
  (7) Designate local maxima as tree tops and use a decision tree method to grow individual crowns around the local maxima. &
  Data collected by ALS in Pellizzano, Trento, Italy; Other output are biomass and carbon density; Data open\tnote{a}; Code not open. &
  \citep{Michele2016Apr5Tree} \\
 &
  (8) Deep learning method to recognize trees and then use height-related gradient information to accomplish individual tree crown delineation. &
  Data collected by UAV LiDAR in Chizhou city, Anhui province, China; Data not open; Code not open. &
  \citep{Chen2021Jan21Individual} \\
 &
  (9) Water expansion controlled by the energy function was applied for accurate crown segmentation. &
  Data collected by UAV LiDAR in Guangxi province, China; Data not open; Code open\tnote{b}. &
  \citep{Yun2021Jan23Individual} \\
 &
  (10) Deep learning object detection algorithm to identify ITCs from the heightmaps generated from point cloud. &
  Data collected by ALS in Nanjing, southeastern China; Data open\tnote{b}; Code not open. &
  \citep{Sun2022Jun14Individual} \\
\hspace*{4em}Sectorial voxelization &
  (11) Detect the 3D symmetrical structure of individual trees to estimate the crown radius and crown base height. &
  Data collected by ALS and TLS in northern Sweden; Data not open; Code not open. &
  \citep{Huo2022Jan3Towards} \\
Single task: individual tree segmentation &
   &
  Main output is pointwise instance ID. &
   \\
\hspace*{4em}Point clustering based &
  (12) Isolate trees individually and sequentially from the point cloud, from the tallest tree to the shortest based on their relative spacing. &
  Data collected by ALS in Sierra Nevada Mountains, California, U.S.; Data not open; Code not open. &
  \citep{Li2012JanNew} \\
 &
  (13) Mean shift segmentation method based on both spatial and multispectral features. &
  Data collected by ALS in Tobermory, Ontario, Canada; Other output is tree position; Data not open; Code not open. &
  \citep{Dai2018Aug17new} \\
 &
  (14) A self-adaptive mean shift tree segmentation method. The bandwidth is acquired by analyzing canopy vertical structures at multiple directions. &
  Data collected by UAV LiDAR in Yancheng city, Jiangsu, China; Other output are tree position and height; Data not open; Code not open. &
  \citep{Yan2020Feb5Self} \\
 &
  (15) Trunk extraction at first. Use distance based clustering for individual tree segmentation. &
  Data collected by TLS in Shangri-La city in northwest Yunnan, China; Data not open; Code not open. &
  \citep{Liu2021Mar4} \\
 &
  (16) Graph based node pathing and clustering. &
  Data collected by TLS in Evo, Finland and Victoria, Australia; Other output are tree location, crown area and volume; Data open; Code not open. &
  \citep{Wang2021Apr3Individual} \\
 &
  (17) Hybrid clustering technique by combining DBSCAN and K-means for segmenting individual trees. &
  Data collected by ALS and UVA LiDAR in Shenmu city, Shaanxi province, China; Data not open; Code not open. &
  \citep{Chen2021Jun14Research} \\
 &
  (18) Hierarchical region-merging based on graph. &
  Data collected by UAV LiDAR in Huanan county, Heilongjiang province, China; Other output are tree position and height; Data not open; Code not open. &
  \citep{Hao2022JanHierarchical} \\
 &
  (19) Super voxel-based hierarchical clustering for street individual tree extraction. &
  Data collected by MLS; Other output is tree position; Data not open; Code not open. &
  \citep{Li2022Jan20branch} \\
 &
  (20) Improved DBSCAN to detect the trunks and obtain the initial clustering results. Use Hough circle fitting method to modify the trunk detection results. Individual tree segmentation based on regional growth layer-by-layer clustering. &
  Data collected by TLS in southwest Germany and China; Other output is tree position; Data open\tnote{a}; Code not open. &
  \citep{Fu2022Apr2Segmenting} \\
 &
  (21) Hierarchical grouping methods based on the cut-pursuit graph algorithm. &
  Data collected by TLS in Finland and Canada; Other output is tree position; Data open\tnote{c}; Code open\tnote{d}. &
  \citep{Xi2022Dec2Graph} \\
 &
  (22) A new topological technique rooted in discrete Morse theory to segment input point clouds into single trees. &
  Data collected by TLS in Sierra National Forest, U.S. and Evo, Finland; Data open; Code not open. &
  \citep{Xu2023JanTopology} \\
\hspace*{4em}DSM or CHM based &
  (23) An improved local maximum method for treetop detection and then inverse operation of the tree climbing method is developed for segmenting individual trees. &
  Data collected by ALS in North Dallas, Texas, U.S.; Other output is tree position, tree height, tree base height, crown depth and crown diameter; Data not open; Code not open. &
  \citep{Zhang2015Jun16Individual} \\
 &
  (24) Coarse segmentation from a marker-controlled watershed segmentation. Combination of a multidirectional 3D profile analysis and K-means clustering is carried out on each point cluster after the coarse segmentation. &
  Data collected by ALS in Cotolivier, Italy and Leskova, Slovenia; Other output are tree height and position; Data open\tnote{c}; Code not open. &
  \citep{Yang2020Mar12Individual} \\
 &
  (25) CHM based method by processing both leaf-on and leaf-off point cloud. &
  Data collected by UAV LiDAR in Liaoning province, northeast China; Other output is tree height; Data open\tnote{b}; Code not open. &
  \citep{Chen2022Jun10Individual} \\
 &
  (26) Similar to (25). &
  Data collected by UAV LiDAR in coastal area of Jiangsu province, China; Other output is tree position; Data not open; Code not open. &
  \citep{Pu2023Mar16New} \\
 &
  (27) Similar to (24). Couple the watershed algorithm with a new clustering algorithm. &
  Data collected by ALS and ULS in Saihanba, China; Other output are tree position and height; Data open; Code open. &
  \citep{Li2023JulIndividual} \\
\hspace*{4em}Deep learning based &
  (28) RandLAnet to remove non tree points. 2D detection based deep learning for tree instance segmentation and post processing refinement. &
  Data collected by TLS in Evo, Finland and Guigang city, Guangxi Zhuang Autonomous Region, China; Other output is tree position, tree height, tree DBH, crown diameter; Data not open; Code not open. &
  \citep{Chang2022Oct6Two} \\
 &
  (29) Top-down instance segmentation deep learning and self-adaptive mean shift clustering. &
  Data collected by ALS in Blue Ridge area of Washington, U.S. and Bretten, Germany; Data open; Code not open. &
  \citep{Zhang2023Jun5Towards} \\
Single task: individual tree component segmentation &
   &
  Main output is pointwise semantic labels. &
   \\
\hspace*{4em}Hand-crafted feature based &
  (30) Graph-structured class regularizations to achieve a spatially smooth classification result. &
  Data collected by TLS in eastern Cameroon; Data open; Code open. &
  \citep{Wang2019Dec9LeWoS} \\
 &
  (31) Design new features for the learning process, which supplements the current geometric features in terms of the topological information. The second local phase designs a new least-cost path model to further separate wood and foliage point. &
  Data collected by TLS in Dongtai forest, Jiangsu province, China; Data not open; Code not open. &
  \citep{Xu2021Jun18Separation} \\
 &
  (32) Classification based on segment-wise geometric features. &
  Data collected by TLS in China; Data open; Code open\tnote{b}. &
  \citep{Wan2021Sep6Novel} \\
\hspace*{4em}Deep learning based &
  (33) FCN for classify wood, branch and others. &
  Data collected by TLS in Canada; Data not open; Code not open. &
  \citep{Xi2018Aug2Filtering} \\
 &
  (34) Classify terrain, vegetation, CWD and stem based on PointNet++. &
  Data collected by TLS, ALS, MLS and UAV-based aerial photogrammetry (UAS\_AP) in Australia and New Zealand; Other output is DTM; Data open\tnote{b}; Code open. &
  \citep{Krisanski2021Apr7Sensor} \\
 &
  (35) Similar to (34). PointNet++ model for segmenting the canopy, trunk, and branches of tree. &
  Data collected by TLS in Korea; Data not open; Code not open. &
  \citep{Kim2023Jun5Automated} \\
 &
  (36) Similar to (34). Leaf-wood separation network. &
  Data collected by TLS in eastern Cameroon; Data open; Code not open. &
  \citep{Jiang2023Jun25LWSNet} \\
\hspace*{4em}Hybrid features based&
  (37) Recurrent Neural Networks (RNNs) that directly estimates the geometric parameters of individual tree stems. &
  Data collected by ALS and TLS in Australia and New Zealand; Data not open; Code not open. &
  \citep{Wang2023Feb13Tree} \\
Multiple tasks &
   &
   &
   \\
 &
  (38)Raster based stem detection. &
  Data collected by TLS in Remningstorp estate, south-western Sweden; Tasks include DEM generation, tree stem detection, tree stem and canopy separation, tree attibutes calculation (DBH, height); Data not open; Code not open. &
  \citep{Olofsson2014May12Tree} \\
 &
  (39)GUI software with source code. &
  Data collected by TLS; Tasks include DTM generation, individual tree segmentation, tree attributes calculation (position, height, DBH, stem profiles and detailed crown parameters); Data open; Code open. &
  \citep{Jan2017May43D} \\
 &
  (40)Step by step methods. At first ground remove; raster based faster RCNN for individual tree segmentation; 3D FCN for stem segmentation. &
  Data collected by TLS in Australia; Tasks include DTM generation, individual tree segmentation, stem points extraction and stem reconstruction; Data not open; Code not open. &
  \citep{Windrim2020May6Detection} \\
 &
  (41)Graph partition and shortest path segmentation and calculate wood probability for each point. &
  Data collected by TLS in synthetic dataset, Evo, Finland and Großgöttfritz, the federal state of Lower Austria; Tasks include individual tree segmentation, leaf-wood classification and tree attributes (crown diameter, height, position); Data open\tnote{a}; Code open. &
  \cite{Wang2020May28Unsupervised} \\
 &
  (42)R package by intigrating existing methods. &
  Data collected by ALS; Tasks include DTM generation, semantic segmentation (building, vegetation, water, power lines, etc.), individual tree segmentation, tree attributes calculation; Data not open; Code open. &
  \citep{Roussel2020Sep24lidR} \\
 &
  (43)Region growing algorithm that starts at the stem voxels and spreads out over the crown. &
  Data collected by TLS in Evo, Finland; Tasks include DTM generation, individual tree detection, tree crown segmentation and tree attributes calculation (stem diameters, height, stem curve, stem volume); Data open; Code not open. &
  \citep{Brolly2021Jan19Voxel} \\
 &
  (44)PointNet++ for semantic segmentation. The remaining vegetation points are assigned to be the same tree as the nearest cylinder measurement in X and Y coordinates. &
  Data collected by TLS in western Australia; Tasks include DTM generation, semantic segmentation (terrain, vegetation, CWD, stems), individual tree segmentation and tree attributes calculation (height, DBH); Data not open; Code open. &
  \citep{Krisanski2021Nov16Forest} \\
  &
  (45)CHM-based watershed segmentation and normalized cut based on spectral and textural features. &
  Data collected by UAV-based LiDAR, and hyperspectral and ultrahigh-resolution RGB data in Shenzhen city, China; Tasks include individual tree segmentation and tree species classification; Data not open; Code not open. &
  \citep{Qin2022Jul6Individual} \\
 &
  (46)PointNet++ semantic segmentation; Graph-based approach for instance segmentation. &
  Data collected by MLS in south-eastern Norway; Tasks include semantic segmentation (vegetation, terrain, and stem, CWD), individual tree segmentation and tree attributes calculation (height); Data not open; Code open. &
  \citep{Wielgosz2023Jul27P2T}\\* \midrule \insertTableNotes
\end{xltabular}
\end{landscape}
\end{ThreePartTable}
}

% ========= OLD COMMENTED VERSION ===========

\begin{comment}
\newpage
{
\tiny
\begin{ThreePartTable}
\begin{TableNotes}
\item[a] Partly available.
\item[b] Contact the author.
\item[c] No pointwise instance ID.
\item[d] Incorporated in CloudCompare software.
\end{TableNotes}

\begin{landscape}
\begin{xltabular}{\textwidth}{p{0.1cm}p{0.3cm}p{0.5cm}p{1.3cm}p{6cm}p{4cm}p{1cm}p{2cm}p{0.5cm}p{0.5cm}p{2.5cm}}
\captionsetup{justification=centering}
\caption{Overview of representative methods for single specific forestry inventory tasks}
\label{tab:ReviewSingleTreeTasks}\\
\toprule
 \multirow{2}{0.1cm}{Task} &
  \multirow{2}{0.3cm}{Main output} &
  \multirow{2}{0.5cm}{Category} &
  \multirow{2}{1.3cm}{Typical methods} &
  \multirow{2}{2.5cm}{Highlight} &
  \multirow{2}{1.6cm}{Study area} &
  \multirow{2}{1cm}{Scanner} &
  \multirow{2}{1.8cm}{Other outputs} &
  \multicolumn{2}{c}{\multirow{1}{*}{Open source}} &
  \multirow{2}{2.5cm}{Similar methods (notes)}  \\* \cmidrule(lr){9-10}
 &
   &
   &
   &
   &
   &
   &
   &
  \multicolumn{1}{c}{Data} &
  \multicolumn{1}{c}{Code} &
   \\* \midrule
\endfirsthead
%
\multicolumn{11}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\toprule
 \multirow{2}{0.1cm}{Task} &
  \multirow{2}{0.3cm}{Main output} &
  \multirow{2}{0.5cm}{Category} &
  \multirow{2}{1.3cm}{Typical methods} &
  \multirow{2}{2.5cm}{Highlight} &
  \multirow{2}{1.6cm}{Study area} &
  \multirow{2}{1cm}{Scanner} &
  \multirow{2}{1.8cm}{Other outputs} &
  \multicolumn{2}{c}{\multirow{1}{*}{Open source}} &
  \multirow{2}{2.5cm}{Similar methods (notes)}  \\* \cmidrule(lr){9-10}
 &
   &
   &
   &
   &
   &
   &
   &
  \multicolumn{1}{c}{Data} &
  \multicolumn{1}{c}{Code} &
   \\* \midrule
\endhead
%
\multicolumn{11}{r}{{Continued on next page}} \\ %\hline
\endfoot
\endlastfoot
%
\multicolumn{1}{c}{\multirow{18}{*}[0ex]{\rotatebox[origin=c]{90}{Individual tree detection}}}
&
  \multicolumn{1}{c}{\multirow{18}{*}[0ex]{\rotatebox[origin=c]{90}{Tree position}}}
  &
  \multirow{9}{0.8cm}{Locate stem center} &
  \citep{Zhang2019Jan16ANovel} &
  Connected component segmentation of stem points &
  - Evo, Finland\newline
  - Beijing, China
  &
  TLS &
  DBH &
  Yes\tnote{a}&
  No &
   \\
   &
   &
   &
  \citep{PaulaPires2022Mar18Individual} &
  Intensity-based point clustering per scanline &
  Southern Sweden &
  - MLS\newline
  - ALS &
  - DBH\newline
  - Stem profiles\newline
  - Stem volume &
  No &
  No &
   \\
   &
   &
   &
  \citep{Zhang2023Feb2ATree} &
  Multiple 2D raster based on height sections &
  Aichi Prefecture, Japan &
  - DLS\newline
  - TLS &
  Tree height &
  No &
  No &
   \\* \cmidrule(l){3-11} 
   &
   &
   \multirow{9}{0.8cm}{Locate crown center} &
  \citep{Zoerner2018Nov13LiDAR} &
  Find local maxima in a CHM as initial tree locations, and accurately identify the tree top positions by combining a raster-based tree crown delineation approach with information from the DSM and DTM &
  Wellington, New Zealand &
  ALS &
  Tree crowns delineation &
  Yes &
  Yes &
  \\
   &
   &
   &
  \citep{Liu2021Mar6Individual} &
  Locate tree position at the clustering center of higher points within a spatial neighborhood, and detect the center by a location-based recursive algorithm &
  - Simulated forest\newline
  - Milwaukee, Wisconsin, United States\newline
  - Denton, Texas, United States &
  ALS &
  \textbackslash &
  No &
  No &
   \\* \midrule
 \multicolumn{1}{c}{\multirow{18}{*}[-0ex]{\rotatebox[origin=c]{90}{Individual tree crown segmentation}}}
&
 \multicolumn{1}{c}{\multirow{18}{*}[-0ex]{\rotatebox[origin=c]{90}{Tree crown delineation/crown width}}}&
  \multirow{13}{0.5cm}{DSM or CHM based} &
  \citep{Strimbu2015Mar18graph} &
  Height raster image based graph partition &
  Vernon Parish, Louisiana, U.S. &
  ALS &
  \textbackslash &
  No &
  No &
   \\
   &
   &
   &
  \citep{Michele2016Apr5Tree} &
  Designate local maxima as tree tops and use a decision tree method to grow individual crowns around the local maxima &
  Pellizzano, Trento, Italy &
  ALS &
  - Biomass\newline
  - Carbon density &
  Yes\tnote{a} &
  No &
   \\
    &
   &
   &
  \citep{Chen2021Jan21Individual} &
  Deep learning method to recognize trees and then use height-related gradient information to accomplish individual tree crown delineation &
  Chizhou City, Anhui province, China &
  UAV LiDAR &
  \textbackslash &
  No &
  No &
   \\
 &
   &
   &
  \citep{Yun2021Jan23Individual} &
  Water expansion controlled by the energy function was applied for accurate crown segmentation &
  Guangxi province, China &
  UAV LiDAR &
  \textbackslash &
  No &
  Yes\tnote{b} &
   \\
 &
   &
   &
  \citep{Sun2022Jun14Individual} &
  Deep learning object detection algorithm to identify ITCs from the heightmaps generated from point cloud &
  Nanjing, in southeastern China &
  ALS &
  \textbackslash &
  Yes\tnote{b} &
  No &
   \\* \cmidrule(l){3-11} 
 &
   &
  \multirow{3}{1cm}{Sectorial voxelization} &
  \citep{Huo2022Jan3Towards} &
  Detects the 3D symmetrical structure of individual trees to estimate the crown radius and crown base height &
  North of Sweden &
  - ALS\newline
  - TLS &
  \textbackslash &
  No &
  No &
   \\ \midrule \pagebreak
   \multicolumn{1}{c}{\multirow{30}{*}[0ex]{\rotatebox[origin=c]{90}{Individual tree segmentation}}}
   &
   \multicolumn{1}{c}{\multirow{30}{*}[0ex]{\rotatebox[origin=c]{90}{Pointwise instance ID}}} &
  \multirow{30}{0.8cm}{Point clustering based} 
   &
  \citep{Li2012JanNew} &
  Isolate trees individually and sequentially from the point cloud, from the tallest tree to the shortest based on their relative spacing &
  Sierra Nevada Mountains, California, U.S. &
  ALS &
  \textbackslash &
  No &
  No &
   \\
   &
   &
   &
  \citep{Dai2018Aug17new} &
  Mean shift segmentation method based on both spatial and multispectral features &
  Tobermory, Ontario, Canada &
  \multirow{1}{1cm}{ALS} &
  Tree position &
  No &
  No &
   \\
   &
   &
   &
  \citep{Yan2020Feb5Self} &
  A self-adaptive mean shift tree segmentation method. The bandwidth is acquired by analyzing canopy vertical structures at multiple directions &
  Yancheng City, Jiangsu, China &
  UAV LiDAR &
  - Tree position\newline
  - Tree height &
  No &
  No &
   \\
   &
   &
   &
  \citep{Chen2021Jun14Research} &
  Hybrid clustering technique by combining DBSCAN and K-means for segmenting individual trees &
  Shenmu city, Shaanxi province, China &
  - ALS\newline
  - UVA LiDAR &
  \textbackslash &
  No &
  No &
   \\
   &
   &
   &
  \citep{Hao2022JanHierarchical} &
  Hierarchical region-merging based on graph &
  Huanan county, Heilongjiang province, China &
  UAV LiDAR &
  - Tree position\newline
  - Tree height &
  No &
  No &
   \\
   &
   &
   &
  \citep{Li2022Jan20branch} &
  Super voxel-based hierarchical clustering for street individual tree extraction &
  \textbackslash &
  MLS &
  Tree position &
  No &
  No &
   \\
   &
   &
   &
  \citep{Fu2022Apr2Segmenting} &
  Improved DBSCAN to detect the trunks and obtain the initial clustering results. Use Hough circle fitting method to modify the trunk detection results. Individual tree segmentation based on regional growth layer-by-layer clustering. &
  - Southwest Germany\newline
  - China &
  TLS &
  Tree position &
  Yes\tnote{a} &
  No &
  \citep{Liu2021Mar4} (Trunk extraction at first. Use distance based clustering for individual tree segmentation. Study area in Shangri-La City in Northwest Yunnan, China.) \\
 &
  &
  &
  \citep{Xi2022Dec2Graph} &
  Hierarchical grouping methods based on the cut-pursuit graph algorithm &
  - Finland\newline
  - Canada &
  TLS &
  Tree position &
  Yes\tnote{c} &
  Yes\tnote{d} &
  \citep{Wang2021Apr3Individual} (Graph based node pathing and clustering. Data available.) \\
 &
   &
   &
  \citep{Xu2023JanTopology} &
  A new topological technique rooted in discrete Morse theory to segment input point clouds into single trees &
  - Sierra National Forest in U.S.\newline
  - Evo, Finland &
  TLS &
  \textbackslash &
  Yes &
  No &
   \\ \cmidrule(l){3-11} \pagebreak
  \multicolumn{1}{c}{\multirow{23}{*}[0ex]{\rotatebox[origin=c]{90}{Individual tree segmentation}}}
   &
   \multicolumn{1}{c}{\multirow{23}{*}[0ex]{\rotatebox[origin=c]{90}{Pointwise instance ID}}} &
  \multirow{16}{0.8cm}{DSM or CHM based} &
  \citep{Zhang2015Jun16Individual} &
  An improved local maximum method for treetop detection and then inverse operation of the tree climbing method is developed for segmenting individual trees &
  North Dallas, Texas, United States &
  ALS &
  - Tree position\newline
  - Tree height\newline
  - Tree base height\newline
  - Crown depth\newline
  - Crown diameter &
  No &
  No &
   \\
   &
   &
   &
  \citep{Yang2020Mar12Individual} &
  Coarse segmentation from a marker-controlled watershed segmentation. Combination of a multidirectional 3D profile analysis and K-means clustering is carried out on each point cluster after the coarse segmentation. &
  - Cotolivier, Italy\newline
  - Leskova, Slovenia &
  ALS &
  - Tree height\newline
  - Tree position &
  Yes\tnote{c} &
  No &
  \citep{Li2023JulIndividual} (Couples the watershed algorithm with a new clustering algorithm. Data and code are both available. Study area in Saihanba, China.) \\
 &
   &
   &
  \citep{Pu2023Mar16New} &
  CHM based method by processing both leaf-on and leaf-off point cloud &
  Coastal area of Jiangsu province, China &
  UAV LiDAR &
  Tree position &
  No &
  No &
  \citep{Chen2022Jun10Individual} (Data is open source\tnote{b}. Study area in Liaoning Province, Northeast China.) \\* \cmidrule(l){3-11} 
 &
   &
  \multirow{7}{0.8cm}{Deep learning based} &
  \citep{Chang2022Oct6Two} &
  Randlanet to remove non tree points. 2D detection based deep learning for tree instance segmentation and post processing refinement. &
  - Evo, Finland\newline
  - Guigang City, Guangxi Zhuang Autonomous Region, China &
  TLS &
  - Crown diameter\newline
  - Tree height\newline
  - Tree position\newline
  - Tree DBH &
  No &
  No &
   \\
 &
   &
   &
  \citep{Zhang2023Jun5Towards} &
  Top-down instance segmentation deep learning and self-adaptive mean shift clustering. &
  - Blue Ridge area of Washington, USA\newline - Bretten, Germany &
  ALS &
  \textbackslash &
  Yes &
  No &
   \\ \midrule \pagebreak
 \multicolumn{1}{c}{\multirow{26}{*}[0ex]{\rotatebox[origin=c]{90}{Wood and foliage separation/Individual tree decomposing}}}
 &
 \multicolumn{1}{c}{\multirow{26}{*}[0ex]{\rotatebox[origin=c]{90}{Pointwise semantic labels}}} &
  \multirow{9}{0.8cm}{Hand-crafted feature based} &
  \citep{Wang2019Dec9LeWoS} &
  Graph-structured class regularizations to achieve a spatially smooth classification result &
  Eastern Cameroon &
  TLS &
  \textbackslash &
  Yes &
  Yes &
   \\
 &
   &
   &
  \citep{Xu2021Jun18Separation} &
  Design new features for the learning process, which supplements the current geometric features in terms of the topological information. The second local phase designs a new least-cost path model to further separate wood and foliage point &
  Dongtai Forest, Jiangsu Province, China &
  TLS &
  \textbackslash &
  No &
  No &
   \\
   &
   &
   &
  \citep{Wan2021Sep6Novel} &
  Classification based on segment-wise geometric features &
  China &
  TLS &
  \textbackslash &
  Yes &
  Yes\tnote{b} &
   \\* \cmidrule(l){3-11} 
 &
   &
  \multirow{13}{0.8cm}{Deep learning based} &
  \citep{Krisanski2021Apr7Sensor} &
  Classify terrain, vegetation, CWD and stem based on PointNet++ &
  - Australia\newline
  - New Zealand &
  - TLS\newline
  - ALS\newline
  - MLS\newline
  - UAV-based aerial photogrammetry (UAS\_AP) &
  DTM &
  Yes\tnote{b} &
  Yes &
  - \citep{Xi2018Aug2Filtering} (FCN for classify wood, branch and others. Study area in Canada)\newline
  - \citep{Kim2023Jun5Automated} (PointNet++ model for segmenting the canopy, trunk, and branches of tree. Study area in Korea.)\newline
  - \citep{Jiang2023Jun25LWSNet} (Leaf-wood separation networks. Study area in eastern Cameroon) \\* \cmidrule(l){3-11} 
 &
   &
  \multirow{4}{0.8cm}{Hybrid features} &
  \citep{Wang2023Feb13Tree} &
  Recurrent Neural Networks (RNNs) that directly estimates the geometric parameters of individual tree stems. &
  - Tumut, NSW, Australia\newline
  - Queensland, Australia\newline
  - Tasmania, Australia\newline
  - Rotorua, New Zealand &
  - ALS\newline
  - TLS &
  \textbackslash &
  No &
  No &
   \\* \bottomrule
\insertTableNotes
\end{xltabular}
\end{landscape}
\end{ThreePartTable}
}
\end{comment}

\begin{comment}
\newpage
{
\tiny
\begin{ThreePartTable}
\begin{TableNotes}
\item[a] Partly available.
\end{TableNotes}

\begin{landscape}
\begin{xltabular}{\textwidth}{p{1.5cm}p{7cm}p{5cm}p{3.5cm}p{0.5cm}p{0.5cm}p{3cm}}
\captionsetup{justification=centering}
\caption{Overview of representative methods for processing multiple forestry inventory tasks}
\label{tab:ReviewMultiTaskMethods}\\
\toprule
\multirow{2}{*}{Methods} &
  \multirow{2}{*}{Tasks} &
  \multirow{2}{*}{Highlights} &
  \multirow{2}{*}{Scanner type} &
  \multicolumn{2}{l}{Open source} &
  \multirow{2}{*}{Study area} \\* \cmidrule(lr){5-6}
 &
   &
   &
   &
  Data &
  Code &
   \\ \midrule
\endfirsthead
%
\multicolumn{7}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\toprule
\multirow{2}{*}{Methods} &
  \multirow{2}{*}{Tasks} &
  \multirow{2}{*}{Highlights} &
  \multirow{2}{*}{Scanner type} &
  \multicolumn{2}{l}{Open source} &
  \multirow{2}{*}{Study area} \\* \cmidrule(lr){5-6}
 &
   &
   &
   &
  Data &
  Code &
   \\ \midrule
\endhead
%
\bottomrule
\endfoot
%
\endlastfoot
%
\citep{Olofsson2014May12Tree} &
  - DEM\newline
  - Tree stem detection\newline
  - Tree stem and tree canopy separation\newline
  - Tree attibutes (DBH, height) &
  Raster based stem detection &
  TLS &
  No &
  No &
  Remningstorp estate, south-western Sweden \\
  \citep{Jan2017May43D} &
  - DTM\newline
  - Individual tree segmentation\newline
  - Tree attributes (position, height, DBH, stem profiles and detailed crown parameters) &
  GUI software with source code &
  TLS &
  Yes &
  Yes &
  \textbackslash \\
\citep{Windrim2020May6Detection} &
  - DTM generation\newline
  - Individual tree segmentation\newline
  - Stem points extraction\newline
  - Stem reconstruction &
  Step by step methods. At first ground remove; raster based faster RCNN for individual tree segmentation; 3D FCN for stem segmentation &
  ALS &
  No &
  No &
  - Tumut, NSW, Australia\newline
  - Carabost, NSW, Australia \\
  \cite{Wang2020May28Unsupervised} &
  - Individual tree segmentation\newline
  - leaf-wood classification\newline
  - Tree attributes(crown diameter, height, position) &
  Graph partition and shortest path segmentation and calculate wood probability for each point &
  TLS &
  Yes\tnote{a} &
  Yes &
  - Synthetic dataset\newline
  - Evo, Finland\newline
  - Großgöttfritz, the federal state of Lower Austria \\
  \citep{Roussel2020Sep24lidR} &
  - DTM\newline
  - Semantic segmentation (building, vegetation, water, power lines, etc.)\newline
  - Individual tree segmentation\newline
  - Tree atrributes &
  R package by intigrating existing methods &
  ALS &
  No &
  Yes &
  \textbackslash \\
  \citep{Brolly2021Jan19Voxel} &
  - DTM\newline
  - Individual tree detection\newline
  - Tree crown segmentation\newline
  - Tree attributes (stem diameters, height, stem curve, stem volume) &
  Region growing algorithm that starts at the stem voxels and spreads out over the crown &
  TLS &
  Yes &
  No &
  Evo, Finland \\
\citep{Krisanski2021Nov16Forest} &
  - DTM\newline
  - Semantic seg: terrain, vegetation, CWD, stems\newline
  - Individual tree segmentation\newline
  - Tree attributes (height, DBH) &
  PointNet++ for semantic segmentation. The remaining vegetation points are assigned to be the same tree as the nearest cylinder measurement in X and Y coordinates. &
  TLS &
  No &
  Yes &
  Western Australia \\
\citep{Qin2022Jul6Individual} &
  - Individual tree segmentation\newline - Tree species classification &
  CHM-based watershed segmentation and normalized cut based on spectral and textural features &
  - UAV-based LiDAR\newline
  - Hyperspectral and ultrahigh-resolution RGB data &
  No &
  No &
  Shenzhen City of southern China \\
 \citep{Wielgosz2023Jul27P2T} &
  - Semantic segmentation (vegetation, terrain, and stem, CWD)\newline
  - Individual tree segmentation\newline
  - Tree attributes (height) &
  PointNet++ semantic segmentation; Graph-based approach for instance segmentation &
  MLS &
  No &
  Yes &
  South-eastern Norway \\* \bottomrule
\insertTableNotes
\end{xltabular}
\end{landscape}
\end{ThreePartTable}
}
\end{comment}
